Unclonable Functional Encryption

In a functional encryption (FE) scheme, a user that holds a ciphertext and a function key can learn the result of applying the function to the plaintext message. Security requires that the user does not learn anything beyond the function evaluation. We extend this notion to the quantum setting by providing definitions and a construction for a quantum functional encryption (QFE) scheme which allows for the evaluation of polynomialy-sized circuits on arbitrary quantum messages. Our construction is built upon quantum garbled circuits [BY22]. We also investigate the relationship of QFE to the seemingly unrelated notion of unclonable encryption (UE) and find that any QFE scheme universally achieves the property of unclonable functional encryption (UFE). In particular we assume the existence of an unclonable encryption scheme with quantum decryption keys which was recently constructed by [AKY24]. Our UFE guarantees that two parties cannot simultaneously recover the correct function outputs using two independently sampled function secret keys. As an application we give the first construction for public-key UE with variable decryption keys. Lastly, we establish a connection between quantum indistinguishability obfuscation (qiO) and quantum functional encryption (QFE); Showing that any multi-input indistinguishability-secure quantum functional encryption scheme unconditionally implies the existence of qiO.

==> 5_UncloneableEncryption.tex <==
\section{Uncloneable Encryption}

\subsection{Definitions}

\subsection{Construction}
We define a family of circuits $\{C_y\}_{y \in \bin^n}$ as follows:
\begin{align*}
    C_y(x,a,\rho) &= \text{Measure } \rho\text{ using measurement operator }M_y\text{ to obtain } b\\
    & \text{if } V(x,y,a,b) = 1 \text{ output 1,b else 0,b}
\end{align*}

\begin{itemize}[align=left,leftmargin=2.8em]
    \item[$\bm{\Keygen(1^\lambda) \rightarrow (\pk,\sk)}$] 
            $$ (\mpk, \msk) \leftarrow \QFE.\Setup(1^\lambda)$$
            Sample $y \leftarrow \bin^n$ and create a function secret key for the circuit $C$:
            $$\sk_{C_y} \leftarrow \QFE.\Keygen(\msk, C_y)$$
            
    \item[$\bm{\Enc(1^\lambda, m \in \bin) \rightarrow \ct}$] \phantom{dsadas}
    \begin{itemize}[align=left,leftmargin=2.8em]
        \item If $m=0$ then sample $x,a \leftarrow \bin^n$ and create a maximally mixed state over n qubits $\rho^B = I/n$. 
        $$ \ct \leftarrow \QFE.\Enc(\mpk, (x,a, \rho^B))$$
        \item If $m=1$ then sample $x \leftarrow \bin^n$ and create n EPR pairs $\rho = \EPR^{\otimes n}$. Let the first qubit of each EPR pair be in register $A$ and the second qubit of each EPR pair be in register $B$. Then perform the measurement $M_a$ on register $\rho^A$ to obtain the outcome $a$. 
        $$ \ct \leftarrow \QFE.\Enc(\mpk, (x,a, \rho^B))$$
    \end{itemize}
    
    \item[$\bm{\Dec(\sk, \ct) \rightarrow m}$] Run $\QFE.\Dec(\sk, \rho^B) \rightarrow m,b$
\end{itemize}


\begin{lemma}
    There is a three player non-local game with players $(A,B,C)$ and Verifier $V$ such that when $(A,B,C)$ share any state before the start of the game and can no longer communicate during the game and $A$ receives challenge $x$ and $B,C$ receive challenge $y$, $A$ replies $a$ and $B,C$ reply $b, c$ the probability that $V(x,a,y,b)=1$ and $V(x,a,y,c)=1$ is negligible. 
\end{lemma}

\begin{lemma}
    Some Lemma about extracting $b$ from an adversary that only successfully guesses 0 or 1.
\end{lemma}



\begin{theorem}
    uncloneable-indistinguisheable secure
\end{theorem}


\begin{proof}\phantom{dsad}
\begin{enumerate}[align=left,leftmargin=2.8em]
    \item First show that is indistinguishable secure, $m=0$ and $m=1$ are indistinguisheable
    \item Then show uncloneability for a message that is $m=1$
    \item since cases are indistinguishable this shows it for both cases?
\end{enumerate}

    Let $(split, B,C)$ be a set of algorithms describing a winning strategy against the uncloneable-indistinguishability game. Then we can construct algorithms $(split^*, A^*, B^*, C^*)$ that win the non-local game with non-negligible probability. 

    Let $split^*$ be defined as follows:
    \begin{enumerate}[align=left,leftmargin=2.8em]
        \item Run $(\mpk, \msk) \leftarrow \QFE.\Setup(1^\lambda)$ 
        \item Create n EPR pairs $\rho = \EPR^{\otimes n}$ and let the state which contains the first qubit of each EPR pair be denoted $\rho^A$ which is given to $A^*$.
        \item Create a ciphertext by sampling $x,a \leftarrow \bin$ and encrypt $\ct \leftarrow \QFE.\Enc(\mpk, (x,a,\rho^B))$.
        \item Run the algorithm $split$ with $\ct$ as input until it outputs two states $\sigma^B, \sigma^C$
        \item Give $\mpk, \msk, \sigma^B$ to $B^*$ and $\mpk, \msk, \sigma^C$ o $C^*$.
    \end{enumerate}

    Let $A^*$ be defined as follows:
    \begin{enumerate}[align=left,leftmargin=2.8em]
        \item Upon receiving the challenge $x$ perform the optimal measurement according to  the non-local game on $\rho^A$ to obtain $a$.
        \item Send $a$ to the verifier.
    \end{enumerate}

    Let $B^*$ and $C^*$ be the same algorithm defined as follows:
    \begin{enumerate}[align=left,leftmargin=2.8em]
        \item Upon receiving the challenge $y$ create the function secret key $\sk_{C_y}$ \item Run the algorithm $B$ on the input $\sigma_B$ and $\sk_{C_y}$ and $C$ on input $\sigma_C$ and $\sk_{C_y}$ respectively. 
        \item Somehow extract $b$ from them.
    \end{enumerate}

    \begin{lemma}
        Let $\{B_i\}_{i \in [t]}$ be a set of subroutines of $B$ where $B_i$ describes the $i-th$ use of the secret key $sk_i$. Then $B$ can be written as a set of unitaries $\{U_i, B_i\}_{i \in [t]}$ and a measurement $M$ such that $B = M \circ U_t \circ B_l(C,\sk_C, \cdot) \circ \cdots \circ U_1 \circ B_1(C,\sk_C, \cdot) \rho$. Then based on the security of functional encryption there exist unitaries $\{B'_i\}_{i \in [t]}$ such that every application of $B_i$ can be replaced by an application of $B'_i$ and a Decryption oracle: $B = M \circ U_t \circ B'_t \circ (\Dec(sk_f,\cdot) \otimes \Id) \circ \cdots \circ U_1 \circ B'_1 \circ (\Dec(sk_f,\cdot) \otimes \Id) \rho$.
    \end{lemma}

    \begin{proof}
        is it true? what if they chose the secret key as a message?
    \end{proof}
    
\end{proof}



==> 5_UncloneableEncryption2.0.tex <==
\section{Uncloneable Encryption}
In this section we show how a QFE scheme can be used to transform a one-time secret-key uncloneable encrpytion scheme with quantum decryption keys into a public-key uncloneable encryption scheme with classical encryption and decryption keys. A similar transformation was shown by~\textcite{TCC:AnaKal21} using classical functional encryption to transform an uncloneable encryption scheme with classical secret keys into a public key scheme. 
\todo{describe AK21 technique more}


Unfortunately we cannot directly apply same technique as \cite{TCC:AnaKal21} since the decryption key needs to be hardcoded in the circuit. In our case the decryption key is a quantum state and our QFE scheme does not support quantum circuits with a quantum description. Instead we encrypt part of n EPR pairs and teleport the quantum decryption keys into the ciphertext. Then we can hardcode the teleportation correction keys into the classical description of the quantum circuit. This introduces a randomization of the function secret key which is why we do not achieve fully fledged uncloneable encryption but only a version where Bob and Charlie obtain decryption keys that come from the same distribution but are not exactly the same. 

This leaves the interesting open question of extending our QFE scheme to a functional encryption scheme that can natively include a quantum state in the description of a quantum circuit. Such a QFE scheme together with our transformation would yield an uncloneable-indistinguishable secure encryption scheme with classical decryption keys which is an important open question. 

\input{2.2_UncloneableEncryption}
\label{qfe:sec:onetimeue}


\subsection{Construction: Public Key Uncloneable Encryption 4.0}


Let $\UEQ = (\Keygen, \Enc, \Dec)$ be a one-time uncloneable encryption scheme for single bit messages with quantum decryption keys and let $\QFE = (\Setup, \Keygen, \Enc, \Dec)$ be a non-adaptive single-query quantum functional encryption scheme. 
%Let $\SKE = (\Keygen, \Enc, \Dec)$ be a symmetric-key encryption scheme with pseudorandom ciphertexts of length $l(\lambda)$.

\begin{comment} --- OLD VERSION WITH SKE ---
    \begin{itemize}[align=left,leftmargin=2.8em]
    \item[$\bm{\Keygen(1^\lambda, r) \rightarrow (|\ek\rangle,\dk)}$] Parse the randomness $r$ as $r = (r_0,r_1)$.
    
    Run $\Setup(1^\lambda,r_0) = (\mpk,\msk)$. Sample a random string $\ct \leftarrow \bin^{l(\lambda)}$ using randomness $r_1$. 
    
    Run $\Keygen(\msk, C_\ct) = \sk_C$ for the following circuit: 
    \begin{align*}
        C_\ct(|\ct_0\rangle, |\ct_1\rangle a_0,b_0,a_1,b_1,c,d, \sk) =& \begin{cases}
         a = a_d, b = b_d\quad \text{if } c = 0\\
         \begin{aligned}
           &\Dec(\ct,\sk) = (a',b')\\
           &a = a', b = b'  
         \end{aligned}      \quad \text{if } c = 1
    \end{cases}\\
    &\text{output } |\dk\rangle = X^a Z^b |\ct_d\rangle
    \end{align*}
    
    \item[$\bm{\Enc(\ek, \msg \in \bin) \rightarrow |\ct\rangle}$] 
    
    Generate one-time encryption keys for the UEQ scheme: $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$
    Generate the same key-pair again: $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$.
    
    Sample keys for the QOTP: $(a_0,b_0) \leftarrow \bin^n,  (a_1,b_1)\leftarrow \bin^n$
    
    Sample $d \in \{0,1\}$.
    
   
    
    If $d = 0$:
    
        Create $|\ct_0\rangle = X^{a_0} Z^{b_0} |\dk_0'\rangle$ and $ |\ct_1\rangle = \Id/2$.
        
If $d = 1$:

        Create $ |\ct_0\rangle = \Id/2$ and $|\ct_1\rangle = X^{a_1} Z^{b_1} |\dk_1'\rangle$.
      
        Create $|\ct_2\rangle =\QFE.\Enc(\mpk, |\ct_0\rangle ,|\ct_1\rangle, a_0,b_0,a_1,b_1, 0,d, 0)$.
        
        Create $|\ct_3\rangle = \UEQ.\Enc(\ek',\msg)$.  
        
        Set $|\ct\rangle = (|\ct_2\rangle, |\ct_3\rangle)$.
    
    \item[$\bm{\Dec(\dk, |\ct\rangle) \rightarrow \msg}$] Parse $|\ct\rangle = (|\ct_2\rangle, |\ct_3\rangle)$, $\dk = \sk_C$

    
    Decrypt $|\dk' \rangle = \QFE.\Dec(\sk_C,|\ct_2\rangle)$. 
    Decrypt $\msg \leftarrow \UEQ.\Dec(|\dk'\rangle, |\ct_3\rangle)$.
\end{itemize}
\end{comment}

\begin{itemize}[align=left,leftmargin=2.8em]
    \item[$\bm{\Keygen(1^\lambda, r) \rightarrow (|\ek\rangle,\dk)}$] Parse the randomness $r$ as $r = (r_0,r_1)$.
    
    Run $\QFE.\Setup(1^\lambda,r_0) = (\mpk,\msk)$. Sample random strings $a,b \leftarrow \bin^{l(\lambda)}$  using randomness $r_1$. 
    
    Run $\QFE.\Keygen(\msk, C_{(a,b)}) = \sk_C$ for the following circuit: 
    \begin{align*}
        C_{(a,b)}(|\ct_0\rangle, |\ct_1\rangle, a_0,b_0,a_1,b_1,c) =&\text{ output } |\dk\rangle = (X^{a_0^*} Z^{b_0^*} \otimes X^{a_1^*} Z^{b_1^*}) |\ct_0\rangle \otimes \ct_1\rangle\\
        &\text{ where } (a_i^*,b_i^*) = \begin{cases}
         a_i^* = a_i, b_i^* = b_i\quad \text{if } c = 0\\
         \begin{aligned}
           &a_i^* = a, b_i^* = b  
         \end{aligned}       \text{if } c = 1
    \end{cases}    
    \end{align*}
    
    
    
    \item[$\bm{\Enc(\ek, \msg \in \bin) \rightarrow |\ct\rangle}$] 
    
    Generate one-time encryption keys for the UEQ scheme: $(\ek',|\dk\rangle) \leftarrow \UEQ.\Keygen(1^\lambda)$
   % Generate the same key-pair again: $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$.
    
    Sample  $(a_0,b_0) \leftarrow \bin^{l(\lambda)},  (a_1,b_1)\leftarrow \bin^{l(\lambda)}$

        Sample $d \leftarrow \bin$
        
        Create $|\ct_d\rangle = X^{a_d} Z^{b_d} 0^\lambda \otimes |\dk\rangle$ and $ |\ct_{1-d}\rangle = X^{a_{1-d}} Z^{b_{1-d}} I/2$, where $I/2$ is the maximally mixed state of size $\lambda + | |\dk\rangle|$. 

        Create $|\ct_2\rangle =\QFE.\Enc(\mpk, |\ct_0\rangle ,|\ct_1\rangle, a_0,b_0,a_1,b_1, 0)$.
        
        Create $|\ct_3\rangle = \UEQ.\Enc(\ek',\msg)$.  
        
        Set $|\ct\rangle = (|\ct_2\rangle, |\ct_3\rangle)$.
    
    \item[$\bm{\Dec(\dk, |\ct\rangle) \rightarrow \msg}$] Parse $|\ct\rangle = (|\ct_2\rangle, |\ct_3\rangle)$ and $\dk = \sk_C$.

    
    Decrypt $\rho_{\dk} = \QFE.\Dec(\sk_C,|\ct_2\rangle)$ and split $\rho_\dk$ into two parts by taking the first half and the second half of the qubits: $\rho_{\dk,0}, \rho_{\dk,1}$. Check $\rho_{\dk,0}$ for validity by taking the first $\lambda$ qubits, measuring them in the computational basis and checking if they are 0, if so set $|\dk'\rangle = \rho_{\dk,0}$, else perform the same check on $\rho_{\dk,1}$ and set $|\dk'\rangle = \rho_{\dk,1}$ if the check succeeded. Output $\bot$ if no check succeeded. 
    
    Decrypt and output $\msg \leftarrow \UEQ.\Dec(|\dk'\rangle, |\ct_3\rangle)$.
\end{itemize}


\begin{theorem}
    The above scheme is a one-time encryption scheme that fulfills indistinguishable-uncloneable security for single bit messages.
\end{theorem}

\begin{proof} 
We prove security via a series of Hybrids.
    \paragraph{Hybrid 0:} This is the experiment as defined in \cref{qfe:def:pkeue}.

    \paragraph{Hybrid 1:} Here we split the Key generation in two algorithms to delay the creation of the decryption key. 

    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Sample $r\leftarrow \bin^\lambda$ and $r', r''\leftarrow \bin^{l(\lambda)}$. Set $r_0 = (r,r')$ and $r_1 = (r,r'')$.
        \item $\ek \leftarrow \Keygen_1(1^\lambda, r)$
        \item $(\msg_0,\msg_1, st) \leftarrow A(1^\lambda, \ek)$ where $|\msg_0|=|\msg_1|=n$
        \item $b \leftarrow \bin$
        \item $|\ct\rangle \leftarrow \Enc(\ek, \msg_b)$
        \item $\rho^{BC} \leftarrow A(|\ct\rangle, st)$
        \item $\dk_0 \leftarrow \Keygen_2(1^\lambda, r_0)$, $\dk_1 \leftarrow \Keygen_2(1^\lambda, r_1)$
        \item $b_B \leftarrow B(\rho^B, \dk_0)$ and $b_C \leftarrow C(\rho^C, \dk_1)$   where $B$ and $C$ are not allowed to communicate. 
    \end{enumerate}
    \begin{itemize}
        \item $\Keygen_1(1^\lambda, r)\rightarrow \ek$: $\Keygen_1$ uses randomness $r$ to run the $\Setup$ of the $\QFE$ scheme to obtain $(\mpk,\msk)$ and ouputs $\ek = \mpk$.
        \item $\Keygen_2(1^\lambda,r_i)\rightarrow \dk$: $\Keygen_2$ uses the first part of the randomness to recreate $(\mpk,\msk)$ und uses the second part of the randomness to sample $(a,b)$ and creates the secret key $\sk_C \leftarrow \QFE.\Keygen(\msk, C_{a,b})$.
    \end{itemize}

    \begin{claim}
        $|p_0 - p_1| =0$ where $p_0$ is the probability that exp=1 in Hybrid 0 and $p_1$ is the probability that exp=1 in Hybrid 1.
    \end{claim}

    \begin{proof}
        This change is only syntactical and therefore the Hybrids are indistinguishable. 
    \end{proof}

    \paragraph{Hybrid 2:} In this Hybrid we change $\Enc$ and $\Keygen_2$ as follows:
    \begin{itemize}
        \item $\Enc(\mpk, \msg)\rightarrow |\ct\rangle$
        \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Create $|\ct_3\rangle$ as before: $|\ct_3\rangle  = \UEQ.\Enc(\ek',\msg)$, $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$, $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$
        \item Sample 2 sets of n EPR pairs $\sigma_0^{AB}$ and $\sigma_1^{AB}$. Let $\sigma_0^A$, $\sigma_1^A$ denote  registers containing the first qubit of each EPR pair and $\sigma_0^B$,$\sigma_1^B$ denote registers containing the second qubit of each EPR pair respectively.  Sample $a_0,b_0,a_1,b_1$ randomly and create the QFE ciphertext 
        $$ |\ct_2\rangle = QFE.\Enc(\mpk,\sigma_0^A, \sigma_1^A, a_0,b_0,a_1,b_1,1)$$.
        
        \item Teleport the key $|\dk_0\rangle$,$|\dk_1\rangle$ through the EPR pairs $\sigma_0^B, \sigma_1^B$ respectively and obtain the teleportation keys $(a_0',b_0'),(a_1',b_1')$.
    \end{enumerate}
    \item Sample $d\leftarrow \bin$ and set $r_0 = (a'_d, b'_d)$ and sample $e \leftarrow \bin$ and set $r_{1} = (a_{e}',b_{e},e)$
.    \item $\Keygen_2(1^\lambda, (r,r_0)) \rightarrow \dk_0$: Create a function secret key for the circuit $C_{(a_d',b_d')}$.
    \item $\Keygen_2(1^\lambda, (r,r_1)) \rightarrow \dk_1$: Create a function secret key for the circuit  $C_{(a_{e}',b_{e}',e)}$.
   
    \end{itemize}

    \begin{claim}
        $|p_1 - p_2| \leq negl(\lambda)$ where $p_1$ is the probability that exp=1 in Hybrid 1 and $p_2$ is the probability that exp=1 in Hybrid 2.
    \end{claim}

    \begin{proof}
    We show that an adversary $\Adv = (A, B, C)$ that can win in Hybrid 1 with a higher probability than in Hybrid 2 can be used to break the special 2-player single query IND-security of the underlying $\QFE$ scheme which we define in \cref{qfe:def:2playerindsecurity}.
    During the reduction both parties $B$ and $C$ will need to obtain independently sampled secret keys for the functional encryption scheme. Since our scheme is only single query secure we cannot allow the adversary to sample two secret keys. Instead we show that if two recipients of a ciphertext don't further communicate they can each receive a functional secret key from the single-query secure QFE scheme. 

    Let $\Adv^* = (A^*,B^*,C^*)$ be the adversary in the 2-player single-query non-adaptive IND-security game against the quantum functional encryption scheme. $A^*$ receives the public key $\mpk$ from the experiment and runs $A$ on input $(1^\lambda, \mpk)$ until $A$ outputs messages $\msg_0,\msg_1$. 
    To create the challenge message $\rho_{\msg^*_0}$ $A$ performs the steps of the honest $\Enc$ algorithm (using randomness $r^*$ for $\UEQ.\Keygen$) without the creation of the $\QFE$ ciphertext. Then $A^*$ sets

    $$\rho_{\msg_0^*} = |\ct_0\rangle\langle \ct_0| \otimes |\ct_1\rangle\langle\ct_1| \otimes |a_0,b_0,a_1,b_1,0\rangle \langle a_0,b_0,a_1,b_1,0|$$ 
    To create the challenge message $\rho_{\msg^*_1}$ $A^*$ performs the steps of $\Enc$ (using the same randomness $r^*$ for $\UEQ.\Keygen$) as in Hybrid 2 without creation of the $\QFE$ ciphertext but with the teleportation. Let $(a'_0,b'_0,a_1',b_1')$ be the resulting teleportation keys. Let $a_0,b_0,a_1,b_1$ be the randomly sampled keys.  Then, $A^*$ sets: 

    $$ \rho_{\msg_1^*} = \sigma_0^A \otimes \sigma_1^A \otimes |a_0,b_0,a_1,b_1,1\rangle\langle a_0,b_0,a_1,b_1,1|$$
    

    Now $A^*$ defines $(\rho_{\msg_0^*}, \rho_{\msg_1^*})$ as challenge messages.
    
    $A^*$ samples $d \leftarrow \lambda$ and defines circuits $C_{(a_d', b_d')}$ and $C_{(a_{1-d}', b_{1-d}')}$. 

    $\A^*$ receives $\rho_{\ct}$ from the experiment finishes the simulation of the experiment by forwarding $(\rho_{\ct}, |\ct_3\rangle)$ to $A$ and receiving $\rho^{BC}$.
    $A^*$ forwards $(\rho^B, C_{(a_d, b_d)}(\rho_{\msg_0^*}))$ to $B^*$ and $(\rho^C, C_{(a_{1-d}', b_{1-d}')}$ to $C^*$. 

    $B^*$ and $C^*$ query the $\Keygen$ oracle on the circuits defined by $A^*$ and obtain $\sk_B$ and $\sk_C$ respectively. 

    The combination of message and key queries is admissible, since 

    $$C_{(a_0, b_0)}(\rho_{\msg_0^*}) = 0^\lambda |\dk\rangle \otimes I/2 = C_{(a_0, b_0)}(\rho_{\msg_1^*}) $$

    and 

    $$C_{(a_1, b_1)}(\rho_{\msg_0^*}) = I/2 \otimes 0^\lambda |\dk\rangle = C_{(a_1, b_1)}(\rho_{\msg_1^*}) $$
    
    and $B^*$ $(C^*)$ has no further internal state. 

    \todo[inline, color=red]{This is not an admissible query since the order of I/2 and dk could be switched. If the decryption key is never output but we directly decrypt the UEQ ciphertext inside the circuit and only output the message this problem should go away}

    Then $B^*$ runs $B$ on input $(\rho_b, \sk_B)$ and $C^*$ runs $C$ on input $(\rho_C, \sk_C)$ and they output whatever $B,C$ output. 

    
    The simulation corresponds to Hybrid 1 if the IND-security experiment for QFE selected $\rho_{m_0^*}$ as challenge message and the simulation corresponds to Hybrid 2 if the IND-security experiment for QFE selected $\rho_{m_1^*}$ as challenge message. 
    Therefore, if the winning probability of $(A,B,C)$ differs non-negligibly, $\Adv^*$ can win the 2-player single-key security of $\QFE$ with non-negligible advantage.      
    \end{proof}

    
    \begin{lemma}
    \label{qfe:lem:reductiontoueq}
        In Hybrid 2 the advantage of $\Adv = (A, B, C)$ is negligible if UEQ is secure.
    \end{lemma}
\begin{proof}
    We show that an adversary that breaks the security of the uncloneable encryption scheme breaks uncloneability of the underlying $\UEQ$ encryption scheme with quantum decryption keys with the same advatage. 

    Let $(A,B,C)$ be an adversary that breaks the security of the uncloneable encryption scheme. Then we can build an adversary $(A^*, B^*, C^*)$ that breaks the security of the $\UEQ$ scheme. Run the $\Keygen_1(1^\lambda)$ algorithm to obtain $\ek$ and run $A$ on input $(1^\lambda, \ek)$. Receive the challenge messages $\msg_0, \msg_1$ from $A$ and forward the messages to the experiment of $\UEQ$. Receive the challenge ciphertext $|\ct\rangle$. 
    
    Build the ciphertext as in Hybrid 2: Sample 2 sets of n EPR pairs $\sigma_0^{AB}$ and $\sigma_1^{AB}$. Let $\sigma_0^A$, $\sigma_1^A$ denote registers containing the first qubit of each EPR pair and $\sigma_0^B$,$\sigma_0^B$ denote registers containing the second qubit of each EPR pair respectively. Create the ciphertext $|\ct' \rangle = \QFE.\Enc(\mpk,\sigma_0^A, \sigma_1^A, a_0,b_0,a_1,b_1,1)$ and send $(|\ct\rangle, |\ct'\rangle)$ to  $A$. 
    
    
    $A$ performs the splitting channel and outputs a state $\rho^{BC}$ which is also the state that $A^*$ defines as it's result of the splitting channel. 
    Now $B^*$ and $C^*$ are activated. They take as input the states $\rho^B, \sigma_0^B$ and $\rho^C, \sigma_1^B$ respectively and each receive a copy of the secret key $|\dk\rangle$ from the experiment. 


    $B^*$ teleports the state $ 0^\lambda \otimes |\dk\rangle$ trough the EPR pairs $\sigma_0^B$ and obtains the teleportation correction keys $a_0,b_0$. He produces the secret key $\dk_B = \QFE.\Keygen(\msk, C_{(a_0,b_0)})$. He runs the adversary $B$ on input $\rho^B$ and the secret key $\dk_B$ and outputs whatever $B^*$ outputs. 

    $C^*$ does the same actions as $B^*$ on his respective EPR pairs. He teleports the state $0^\lambda \otimes |\dk\rangle$ trough the EPR pairs $\sigma_1^B$. He obtains the teleportation correction keys $a_1,b_1$ and produces the secret key $\dk_C = \QFE.\Keygen(\msk, C_{(a_1,b_1)})$. He runs the adversary $C$ on input $\rho^C$ and the secret key $\dk_C$ and outputs whatever $C^*$ outputs. 
    
    $(A^*, B^*, C^*)$ wins with the same probability as $(A,B,C)$. 
\end{proof}
\end{proof}


\subsubsection{Special 2-plyaer security of QFE}

In the experiment we  create two copies of the quantum ciphertext. This might not be physically possible since a quantum message is encrypted. This definition only strengthens the security notion and is the most general, e.g. the security notion is also applicable if A has to split the ciphertext into two states before B and C are activated.

\begin{definition}[2-player Single-Query IND-Security for QFE]
\label{qfe:def:2playerindsecurity}

Let $\lambda$ be the security parameter and let $\Adv = (A,B,C)$ be a QPT adversary.
   \begin{align*}
            &\Exp^{2P-IND}_{\Adv,b}(1^\lambda)\\
            &(\mpk,\msk) \leftarrow \Setup(1^\lambda)\\
            %\Adv can make a query to obtain \sk_f
             &(\rho_{\msg_0}, \rho_{\msg_1}, \rho_{\st_B}, \rho_{\st_C}) \leftarrow A(\mpk)\\
             %, \text{where $\rho_{\msg_0}$ and $\rho_{\msg_1}$ are admissible queries} \\ &\text{for the circuit $C$ that $\Adv$ queries. }\\ 
            &\rho_\ct^{\otimes 2} \leftarrow \Enc(\mpk, \rho_{\msg_b})\\
            & b_B \leftarrow B^{O(\cdot)}(\mpk, \rho_\ct, \rho_{\st_B})\\
            & b_C \leftarrow C^{O(\cdot)}(\mpk, \rho_\ct, \rho_{\st_C})
    \end{align*}
The FE scheme is called secure if for any adversary $\Adv = (A,B,C)$ where $B$ and $C$ each make at most one call to $O(\cdot) = \Keygen(\msk, \cdot)$ such that each query individually is an admissible query (\cref{qfe:def:admis}) taking into account the circuit, the challenge messages and either the state $\rho_{\st_B}$ or $\rho_{\st_C}$ it holds that
$$\Pr\left[ b_B = b_C = b \right] \leq \frac{1}{2} + negl(\lambda)$$
where the random coins are taken over the randomness of $\Adv$, $\Setup, \Keygen$ and $\Enc$.
\end{definition}

\begin{lemma}
    Any adaptively IND-secure single-query QFE scheme (\cref{qfe:def:indsecurity}) is also a 2-player single-query IND secure QFE scheme (\cref{qfe:def:2playerindsecurity}).
\end{lemma}

\begin{proof}
    An adversary $\Tilde{A}$ in the single-query QFE IND-experiment can execute an adversary $(A,B,C)$ that wins the 2-player IND-experiment by only executing $A$ and $B$. Since to break security in the 2-player IND-security experiment both players $B$ and $C$ need to guess the correct bit $b$, $\Tilde{A}$ can win the IND-security experiment with the same probability as $(A,B,C)$ wins by outputting the guess $B$ outputs. 
\end{proof}

\begin{remark}
    One could obtain a similar security notion from the weaker version of non-adaptively secure QFE by having $A$ specify two circuits $C_B$ and $C_C$ for which $B$ and $C$ obtain the function secret keys. 
\end{remark}
\begin{comment}

\subsection{Construction: Public Key Uncloneable Encryption}


\begin{definition} (Uncloneable-Indistinguishable Security for Public Key Uncloneable Encryption with Variable Decryption Keys -----NEW------)
\label{qfe:def:pkeue}

        Let $\Adv = (A,B,C)$ be a QPT adversary in the uncloneable-indistinguishable security experiment $\Exp^{UE-VDK}_\Adv$.\\
        
        $\Exp^{UE-VDK}_{\Adv,b}$
    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item $(\ek,\dk_0) \leftarrow \Keygen(1^\lambda, r_0)$, $(\ek,\dk_1) \leftarrow \Keygen(1^\lambda, r_1)$, where $r_0 = (r,r_0',0)$, $r_1 = (r,r_1',1)$, $r_0',r_1' \leftarrow \bin^{l(\lambda)}$, $r \leftarrow \bin^{k(\lambda)}$
        \item $(\msg_0,\msg_1, \rho_\st) \leftarrow A(1^\lambda, \ek)$ where $|\msg_0|=|\msg_1|=n$
        \item $|\ct\rangle \leftarrow \Enc(\ek, \msg_b)$
        \item $\rho^{BC} \leftarrow A(|\ct\rangle, \rho_\st)$
        \item $b_B \leftarrow B(\rho^B, \dk_0)$ and $b_C \leftarrow C(\rho^C, \dk_1)$   where $B$ and $C$ are not allowed to communicate. 
    \end{enumerate}
  
    
     An uncloneable encryption scheme is called one-time uncloneable-indisintguishable secure if for all $(A,B,C)$ there exists a negligible function negl such that for all $\lambda \in \N$: 
    $$\Pr[b_B = b_C = b] \leq \frac{1}{2} + negl(\lambda)$$
\end{definition}


Let $\UEQ = (\Keygen, \Enc, \Dec)$ be a one-time uncloneable encryption scheme for single bit messages with quantum decryption keys and pseudodeterministic $\Keygen$ which takes as input $1^{r(\lambda)}$ bits of randomness and outputs decryption keys in $D(\Hilb_{l(\lambda)})$. Let $\QFE = (\Setup, \Keygen, \Enc, \Dec)$ be a non-adaptive single-query quantum functional encryption scheme. 


\begin{itemize}[align=left,leftmargin=2.8em]
    \item[$\bm{\Keygen(1^\lambda, r) \rightarrow (\ek,\dk)}$] 
    Parse the randomness $r$ as $r = (r_0, r_1, r_2)$.
    
       Run $\QFE.\Setup(1^\lambda,r_0) = (\mpk_0,\msk_0)$. 
       
    Run $\QFE.\Setup(1^\lambda,r_1) = (\mpk_1,\msk_1)$. 
   
    Parse randomness $r_2$ as $(a_0,b_0,a_1,b_1,d)$, where $|a_0|=|a_1|=|b_0|=|b_1| = l(\lambda)$ and $d \in \bin$.
    
    Run $\QFE.\Keygen(\msk_0, C_{(a_0,b_0)}) = \sk_{C_0}$ and
     $\QFE.\Keygen(\msk_1, C_{(a_1,b_1)}) = \sk_{C_1}$ where the circuit $C_{(a,b)}$ is defined as follows:
    
    \begin{align*}
        C_{(a,b)}(|\ct\rangle, a^*,b^*,c) =&\text{ output } |\dk\rangle = X^{a'} Z^{b'} |\ct\rangle\\
        &\text{ where } (a',b') = \begin{cases}
         a' = a^*, b' = b^*\quad \text{if } c = 0\\
         \begin{aligned}
           &a' = a, b' = b  
         \end{aligned}      \quad \text{if } c = 1
    \end{cases}    
    \end{align*}
   % Sample $d \leftarrow \bin$.
    
    Output $(\ek = (\mpk_0,\mpk_1), \dk = (\sk_{C_d},d))$
    
    \item[$\bm{\Enc(\ek, \msg \in \bin) \rightarrow |\ct\rangle}$] 
    
    Generate one-time encryption keys for the UEQ scheme: $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$, where $r \in 1^{r(\lambda)}$.
    Generate the same key-pair again: $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$, s.t. $|\dk_0\rangle = |\dk_1\rangle$.
    
    Sample  $(a_0,b_0) \leftarrow \bin^{l(\lambda)},  (a_1,b_1)\leftarrow \bin^{l(\lambda)}$
    

        Create $|\ct_0\rangle =\QFE.\Enc(\mpk_0, X^{a_0} Z^{b_0}|\dk_0\rangle, a_0,b_0, 0)$.
        
        Create $|\ct_1\rangle =\QFE.\Enc(\mpk_1, X^{a_1} Z^{b_1}|\dk_1\rangle, a_1,b_1, 0)$.
        
        Create $|\ct_3\rangle = \UEQ.\Enc(\ek',\msg)$.  
        
        Set $|\ct\rangle = (|\ct_0\rangle,|\ct_1\rangle, |\ct_3\rangle)$.
    
    \item[$\bm{\Dec(\dk, |\ct\rangle) \rightarrow \msg}$] Parse $|\ct\rangle = (|\ct_0\rangle,|\ct_1\rangle, |\ct_3\rangle)$ and $\dk = (\sk_C,d)$.

    
    Decrypt $|\dk' \rangle = \QFE.\Dec(\sk_C,|\ct_d\rangle)$. 
    Decrypt $\msg \leftarrow \UEQ.\Dec(|\dk'\rangle, |\ct_3\rangle)$.
\end{itemize}


\begin{theorem}
    The above scheme is a public-key uncloneable encryption scheme that fulfills indistinguishable-uncloneable (\cref{qfe:def:pkeue}) security for single bit messages.
\end{theorem}

\begin{proof} 
We prove security via a series of Hybrids.
    \paragraph{Hybrid 0:} This is the experiment as defined in \cref{qfe:def:pkeue}.
    

    \paragraph{Hybrid 1:} Here we split the Key generation in two algorithms to delay the creation of the decryption key. 

    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Sample $r\leftarrow \bin^{2k(\lambda)}$ and $r', r''\leftarrow \bin^{4l(\lambda)}$. Set $r_0 = (r,r',0)$ and $r_1 = (r,r'',0)$.
        \item $\ek \leftarrow \Keygen_1(1^\lambda, r)$
        \item $(\msg_0,\msg_1, st) \leftarrow A(1^\lambda, \ek)$ where $|\msg_0|=|\msg_1|=n$
        \item $|\ct\rangle \leftarrow \Enc(\ek, \msg_b)$
        \item $\rho^{BC} \leftarrow A(|\ct\rangle, st)$
        \item $\dk_0 \leftarrow \Keygen_2(1^\lambda, r_0)$, $\dk_1 \leftarrow \Keygen_2(1^\lambda, r_1)$
        \item $b_B \leftarrow B(\rho^B, \dk_0)$ and $b_C \leftarrow C(\rho^C, \dk_1)$   where $B$ and $C$ are not allowed to communicate. 
    \end{enumerate}
    Concretely in our scheme we split the algorithm as follows:
    
    \begin{itemize}
        \item $\Keygen_1(1^\lambda, r)\rightarrow \ek$: $\Keygen_1$ uses randomness $r = (r_0,r_1)$ to run the $\Setup$ of the $\QFE$ scheme to obtain $(\mpk_0, \mpk_1,\msk_0,\msk_1)$ and outputs $\ek = (\mpk_0,\mpk_1)$.
        \item $\Keygen_2(1^\lambda,r_i)\rightarrow \dk$: $\Keygen_2$ uses the first part of the randomness to recreate $(\mpk_0, \mpk_1,\msk_0, \msk_1)$ and uses the second part of the randomness to define $(a_0,a_0,b_0,b_1,d)$ and creates the secret key $\sk_C \leftarrow \QFE.\Keygen(\msk, C_{a_d,b_d})$.
    \end{itemize}

    \begin{claim}
        Hybrid 0 and Hybrid 1 are perfectly indistinguishable.
    \end{claim}
    \begin{proof}
            This change is only syntactical and therefore the Hybrids are indistinguishable. 
    \end{proof}

    \paragraph{Hybrid 2:} In this Hybrid we change the encryption of $|\ct_0\rangle$ and the creation of $\dk_0$ as follows:
    \begin{itemize}
        \item $\Enc(\mpk, \msg)\rightarrow |\ct_\rangle$
        \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Create $|\ct_3\rangle$ as before: $|\ct_3\rangle  = \UEQ.\Enc(\ek',\msg)$, $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$, $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$
        \item Sample $l(\lambda)$ EPR pairs $\sigma^{AB}$. Let $\sigma^A$  denote  registers containing the first qubit of each EPR pair and $\sigma^B$ denote registers containing the second qubit of each EPR pair respectively.  Sample $a_0,b_0,a_1,b_1$ randomly and create the QFE ciphertexts 
        $$ |\ct_0\rangle = \QFE.\Enc(\mpk_0,\sigma_0^A,a_0,b_0,1)$$.
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk_1,X^{a_1} Z^{b_1} |\dk_1\rangle ,a_1,b_1,0)$$.
        
        
        \item Teleport the key $|\dk_0\rangle$ through the EPR pairs $\sigma^B$ and obtain the teleportation keys $(a_0',b_0')$ and sample $(a_1',b_1')$ randomly.
    \end{enumerate}
    \item Set $r_0 = (a'_0, b'_0, a_1',b_1',0)$ and set $r_{1} = (a_0,b_0,a_{1}',b_{1},1)$
.    \item $\Keygen_2(1^\lambda, (r,r_0)) \rightarrow \dk_0$: Create a function secret key for the circuit $C_{(a_0',b_0')}$.
    \item $\Keygen_2(1^\lambda, (r,r_1)) \rightarrow \dk_1$: Create a function secret key for the circuit  $C_{(a_{1}',b_{1}')}$.
    \todo{this means that B and C definitely get different decryption keys in this Hybrid but in the original experiment they could get the same sometimes.\\ Need to redefine the security definition to make them get different secret keys every time? This issue would also appear in the old construction since in the final Hybrid they always get different keys}
    \end{itemize}

    \begin{claim}
    \label{qfe:claim:hyb2qfered}
         Hybrid 1 and Hybrid 2 are computationally indistinguishable due to the single-key non-adaptive security of QFE. 
    \end{claim}

   \begin{proof}
       
  

    We show that an adversary $\Adv = (A, B, C)$ that can distinguish Hybrid 1 and Hybrid 2 can be used to break the security of the underlying $\QFE$ scheme. 

    Let $\Adv^*$ be the adversary in the single-query non-adaptive IND-security game (\cref{qfe:def:indsecurity}) against the quantum functional encryption scheme. $\Adv^*$ receives one public key $\mpk_0$ from the experiment creates the setup of the second QFE scheme $(\mpk_1, \msk_1) \leftarrow \QFE.\Setup(1^\lambda)$ and runs $A$ on input $(1^\lambda, (\mpk_0, \mpk_1))$ until $A$ outputs messages $\msg_0,\msg_1$. 
    To create the challenge message $\rho_{\msg^*_0}$ $\Adv^*$ performs the steps of the honest $\Enc$ algorithm (using randomness $r^*$ for $\UEQ.\Keygen$) without the creation of the $\QFE$ ciphertext $|\ct_0\rangle$. Then $\Adv^*$ sets

    $$\rho_{\msg_0^*} = X^{a_0} Z^{b_0} |\dk_0\rangle \otimes |a_0,b_0,0\rangle \langle a_0,b_0,0|$$ 
    To create the challenge message $\rho_{\msg^*_1}$ $\Adv^*$ performs the steps of $\Enc$ (using the same randomness $r^*$ for $\UEQ.\Keygen$ to recreate $|\dk_0\rangle$) as in Hybrid 2 without creation of the $\QFE$ ciphertext. That means $\Adv^*$ creates $l(\lambda)$ EPR pairs $\sigma^{AB}$ and teleports $\dk_0\rangle$ trough $\sigma^B$. Let $(a'_0,b'_0)$ be the resulting teleportation keys. Then, $\Adv^*$ sets: 

    $$ \rho_{\msg_1^*} = \sigma_0^A \otimes |a_0,b_0,1\rangle\langle a_0,b_0,1|$$

    Note that in this message the flag bit $c$ is set to $1$.
    Now $\Adv^*$ defines $(\rho_{\msg_0^*}, \rho_{\msg_1^*})$ as challenge messages. 
    $\Adv^*$ requests a function secret key $\sk_C$ for the circuit $C_{(a'_0, b'_0)}$. The combination of message and key queries is an admissible query, since 

    $$C_{(a'_0, b'_0)}(\rho_{\msg_0^*}) = |\dk_0\rangle = C_{(a'_0, b'_0)}(\rho_{\msg_1^*}) $$
    and $\Adv^*$ is not entangled with the state. 

    $\Adv^*$ receives $\rho_{\ct}$ from the experiment finishes the simulation of the experiment by forwarding $(\rho_{\ct}, |\ct_2\rangle, |\ct_3\rangle)$ to $A$, where $|\ct_2\rangle$ and $|\ct_3\rangle$ are created as in the honest encryption algorithm, Hybrid 1 and Hybrid 2 do not differ in this aspect. Then $\Adv^*$ creates the secret key $\sk_{C_1} \leftarrow \QFE.\Keygen(1^\lambda, \msk_1, C_{(a_1,b_1)})$ for random $a,b \leftarrow \bin^{l(\lambda)}$. $\Adv^*$ receives $\rho^{BC}$, forwards $(\rho^B,\sk_C)$ to $B$ and $(\rho^C, \sk_{C_1})$ to $C$. The simulation corresponds to Hybrid 1 if the IND-security experiment for QFE selected $\rho_{m_0^*}$ as challenge message and the simulation corresponds to Hybrid 2 if the IND-security experiment for QFE selected $\rho_{m_1^*}$ as challenge message. Therefore, if $(A,B,C)$ can distinguish the Hybrids, $\Adv^*$ can break the non-adaptive single-key security of $\QFE$.
 \end{proof}

    \paragraph{Hybrid 3:} In this Hybrid we change the encryption of $|\ct_1\rangle$ and the creation of $\dk_1$ as follows:
    \begin{itemize}
        \item $\Enc(\mpk, \msg)\rightarrow |\ct_\rangle$
        \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Create $|\ct_3\rangle$ as before: $|\ct_3\rangle  = \UEQ.\Enc(\ek',\msg)$, $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$, $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$
        \item Sample $l(\lambda)$ EPR pairs $\sigma^{AB}$. Let $\sigma^A$  denote  registers containing the first qubit of each EPR pair and $\sigma^B$ denote registers containing the second qubit of each EPR pair respectively.  Sample $a_1,b_1$ randomly and create the QFE ciphertext 
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk,\sigma_1^A,a_1,b_1,1)$$.
        \item Create $|\ct_0\rangle$ as in Hybrid 2.% which gives $(a_0',b_0')$ .
        
        
        \item Teleport the key $|\dk_1\rangle$ through the EPR pairs $\sigma^B$ and obtain the teleportation keys $(a_1',b_1')$.
    \end{enumerate}
    \item Set $r_{1} = (a_0,b_0,a_{1}',b'_{1},1)$ for $a_0,b_0 \leftarrow \bin^{l(\lambda)}$.
    \item $\Keygen_2(1^\lambda, (r,r_1)) \rightarrow \dk_1$: Create a function secret key for the circuit  $C_{(a_{1}',b_{1}')}$.
    \item Create $|\dk_0\rangle$ as in Hybrid 2.
    
    \end{itemize}
    

    \begin{claim}
        Hybrid 2 and Hybrid 3 are computationally indistinguishable due to the single-key non-adaptive security of QFE.
    \end{claim} 
    \begin{proof}
        The proof follows the same argument as the proof for the previous claim so we omit it here.
    \end{proof}
    
    
    \begin{lemma}
        In Hybrid 3 the advantage of $\Adv = (A, B, C)$ is negligible if UEQ fulfills uncloneable security for UE schemes with quantum decryption keys (\cref{qfe:def:ueqsec}).
    \end{lemma}
\begin{proof}
    We show that an adversary that breaks the security of the uncloneable encryption scheme breaks uncloneability of the underlying $\UEQ$ encryption scheme with quantum decryption keys with the same advatage. 

    Let $(A,B,C)$ be an adversary that breaks the security of the uncloneable encryption scheme. Then we can build an adversary $(A^*, B^*, C^*)$ that breaks the security of the $\UEQ$ scheme. Run the $\Keygen_1(1^\lambda)$ algorithm to obtain $\ek$  and run $A$ on input $(1^\lambda, \ek)$. Receive the challenge messages $\msg_0, \msg_1$ from $A$ and forward the messages to the experiment of $\UEQ$. Receive the challenge ciphertext $|\ct\rangle$. 
    
    Build the ciphertext as in Hybrid 3: Sample 2 sets of n EPR pairs $\sigma_0^{AB}$ and $\sigma_1^{AB}$. Let $\sigma_0^A$, $\sigma_1^A$ denote registers containing the first qubit of each EPR pair and $\sigma_0^B$,$\sigma_0^B$ denote registers containing the second qubit of each EPR pair respectively. Sample $a_0,b_0,a_1,b_1 \leftarrow \bin^{l(\lambda)}$ and create the ciphertexts 
    
    $$|\ct_0 \rangle = \QFE.\Enc(\mpk,\sigma_0^A, a_0,b_0,1)$$ 
    $$|\ct_1 \rangle = \QFE.\Enc(\mpk,\sigma_1^A, a_1,b_1,1) $$
    
    and send $(|\ct_0\rangle, |\ct_1\rangle, |\ct\rangle)$ to  $A$. 
    
    
    $A$ performs the splitting channel and outputs a state $\rho^{BC}$ which is also the state that $A^*$ defines as it's result of the splitting channel. 
    Now $B^*$ and $C^*$ are activated. They take as input the states ($\rho^B, \sigma_0^B$) and ($\rho^C, \sigma_1^B$) respectively and each receive a copy of the secret key $|\dk\rangle$ from the experiment. 


    $B^*$ teleports the state $|\dk\rangle$ trough the EPR pairs $\sigma_0^B$ and obtains the teleportation correction keys $a'_0,b'_0$. He produces the secret key $\dk_B = \QFE.\Keygen(\msk, C_{(a'_0,b'_0)})$. He runs the adversary $B$ on input $\rho^B$ and the secret key ($\dk_B$,0) and outputs whatever $B^*$ outputs. 

    $C^*$ does the same actions as $B^*$ on his respective EPR pairs. He teleports the state $|\dk\rangle$ trough the EPR pairs $\sigma_1^B$. He obtains the teleportation correction keys $a'_1,b'_1$ and produces the secret key $\dk_C = \QFE.\Keygen(\msk, C_{(a'_1,b'_1)})$. He runs the adversary $C$ on input $\rho^C$ and the secret key ($\dk_C$,1) and outputs whatever $C^*$ outputs. \todo{In the final step B and C always receive different decryption keys, so we have to do this in each Hybrid (?)}
    
    $(A^*, B^*, C^*)$ wins with the same probability as $(A,B,C)$. 
\end{proof}
\end{proof}

\paragraph{Remark} Can we use \cite{HKNY23} to make the single bit uncloneable encryption scheme into a multi-bit uncloneable encryption scheme?. \todo{They say (page 10): 'Without loss of generality, we can assume that the secret key sk generated by Unclone.KeyGen(1λ) is uniformly randomly sampled and |sk| = |CT| = λ for all security parameters λ.' But we dont really have that?\\
Furthermore they only prove for secret-key uncloneable encryption but they say it works for public-key uncloneable encryption too}

\paragraph{Remark} Mention that the independently sampled decryption keys security notion is still useful for public key quantum money.

\subsection{Construction: Public Key Uncloneable Encryption  3.0}


\begin{definition} (Uncloneable-Indistinguishable Security for Public Key Uncloneable Encryption with Variable Decryption Keys)
\todo{Is this the desired notion?}
\label{qfe:def:pkeue}

        Let $\Adv = (A,B,C)$ be a QPT adversary in the uncloneable-indistinguishable security experiment $\Exp^{UE-VDK}_\Adv$.\\
        
        $\Exp^{UE-VDK}_{\Adv,b}$
    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item $(\ek,\dk_0) \leftarrow \Keygen(1^\lambda, r_0)$, $(\ek,\dk_1) \leftarrow \Keygen(1^\lambda, r_1)$, where $r_0 = (r,r_0')$, $r_1 = (r,r_1')$, $r_0',r_1' \leftarrow \bin^{l(\lambda)}$, $r \leftarrow \bin^{k(\lambda)}$
        \item $(\msg_0,\msg_1, \rho_\st) \leftarrow A(1^\lambda, \ek)$ where $|\msg_0|=|\msg_1|=n$
        \item $|\ct\rangle \leftarrow \Enc(\ek, \msg_b)$
        \item $\rho^{BC} \leftarrow A(|\ct\rangle, \rho_\st)$
        \item Sample $d\leftarrow\bin$
        \item $b_B \leftarrow B(\rho^B, \dk_d)$ and $b_C \leftarrow C(\rho^C, \dk_{1-d})$   where $B$ and $C$ are not allowed to communicate. 
    \end{enumerate}
  
    
     An uncloneable encryption scheme is called one-time uncloneable-indisintguishable secure if for all $(A,B,C)$ there exists a negligible function negl such that for all $\lambda \in \N$: 
    $$\Pr[b_B = b_C = b] \leq \frac{1}{2} + negl(\lambda)$$
\end{definition}


Let $\UEQ = (\Keygen, \Enc, \Dec)$ be a one-time uncloneable encryption scheme for single bit messages with quantum decryption keys and pseudodeterministic $\Keygen$ which takes as input $1^{r(\lambda)}$ bits of randomness and outputs decryption keys in $D(\Hilb_{l(\lambda)})$. Let $\QFE = (\Setup, \Keygen, \Enc, \Dec)$ be a non-adaptive single-query quantum functional encryption scheme. 


\begin{itemize}[align=left,leftmargin=2.8em]
    \item[$\bm{\Keygen(1^\lambda, r) \rightarrow (\ek,\dk)}$] 
    Parse the randomness $r$ as $r = (r_0, r_1, r_2)$.
    
       Run $\QFE.\Setup(1^\lambda,r_0) = (\mpk_0,\msk_0)$. 
       
    Run $\QFE.\Setup(1^\lambda,r_1) = (\mpk_1,\msk_1)$. 
   
    Parse randomness $r_2$ as $(a,b)$, where $|a_0|=|a_1| = l(\lambda)$.
    
    Run $\QFE.\Keygen(\msk_0, C_{(a,b)}) = \sk_{C_0}$ and
     $\QFE.\Keygen(\msk_1, C_{(a,b)}) = \sk_{C_1}$ where the circuit $C_{(a,b)}$ is defined as follows:
    
    \begin{align*}
        C_{(a,b)}(|\ct\rangle, a^*,b^*,c) =&\text{ output } |\dk\rangle = X^{a'} Z^{b'} |\ct\rangle\\
        &\text{ where } (a',b') = \begin{cases}
         a' = a^*, b' = b^*\quad \text{if } c = 0\\
         \begin{aligned}
           &a' = a, b' = b  
         \end{aligned}      \quad \text{if } c = 1
    \end{cases}    
    \end{align*}
   % Sample $d \leftarrow \bin$.
    
    Output $(\ek = (\mpk_0,\mpk_1), \dk = (\sk_{C_0},\sk_{C_0}))$
    
    \item[$\bm{\Enc(\ek, \msg \in \bin) \rightarrow |\ct\rangle}$] 
    
    Generate a one-time encryption key pair for the UEQ scheme: $(\ek',|\dk\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$, where $r \in 1^{r(\lambda)}$.
    %Generate the same key-pair again: $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r)$, s.t. $|\dk_0\rangle = |\dk_1\rangle$.
    
    Sample  $(a_0,b_0) \leftarrow \bin^{l(\lambda)+ \lambda},  (a_1,b_1)\leftarrow \bin^{l(\lambda)+\lambda}$.
    
    Sample $d \leftarrow \bin$.

    
        Create $|\ct_d\rangle =\QFE.\Enc(\mpk_d, X^{a_d} Z^{b_d} |0\rangle^{\otimes \lambda}|\dk\rangle, a_d,b_d, 0)$. 
        
        Create $|\ct_{1-d}\rangle =\QFE.\Enc(\mpk_{1-d}, I/2, a_{1-d},b_{1-d}, 0)$ where $I/2$ is the maximally mixed state of dimension $l(\lambda)+ \lambda$.
        
        Create $|\ct_3\rangle = \UEQ.\Enc(\ek',\msg)$.  
        
        Set $|\ct\rangle = (|\ct_0\rangle,|\ct_1\rangle, |\ct_3\rangle)$. 
    
    \item[$\bm{\Dec(\dk, |\ct\rangle) \rightarrow \msg}$] Parse $|\ct\rangle = (|\ct_0\rangle,|\ct_1\rangle, |\ct_3\rangle)$ and $\dk = (\sk_{C_0},\sk_{C_1})$.

    
    Decrypt $|\dk_0 \rangle = \QFE.\Dec(\sk_{C_0},|\ct_0\rangle)$ and  decrypt $|\dk_1 \rangle = \QFE.\Dec(\sk_{C_1},|\ct_1\rangle)$.

    If the first $\lambda$ qubits of $|\dk_0 \rangle$ measured in the computational basis are 0, remove the 0 bits from $|\dk_0 \rangle$ and set $|\dk'\rangle = |\dk_0 \rangle$. Else check if the first $\lambda$ qubits of $|\dk_1 \rangle$ measured in the computational basis are 0, if so remove the 0 bits from $|\dk_1\rangle$ and set $|\dk'\rangle = |\dk_1 \rangle$. If neither of the checks succeeded output $\bot$.
    
    Decrypt $\msg \leftarrow \UEQ.\Dec(|\dk'\rangle, |\ct_3\rangle)$ and output $\msg$.
\end{itemize}


\begin{theorem}
    There is a public-key uncloneable encryption scheme that fulfills indistinguishable-uncloneable  security with variable secret keys (\cref{qfe:def:pkeue}) for single bit messages.
\end{theorem}

\begin{proof} 
We prove security via a series of Hybrids.
    \paragraph{Hybrid 0:} This is the experiment as defined in \cref{qfe:def:pkeue}.
    

    \paragraph{Hybrid 1:} Here we split the Key generation in two algorithms to delay the creation of the decryption key. 

    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Sample $r\leftarrow \bin^{2k(\lambda)}$ and $r', r''\leftarrow \bin^{4l(\lambda)}$. Set $r_0 = (r,r')$ and $r_1 = (r,r'')$.
        \item $\ek \leftarrow \Keygen_1(1^\lambda, r)$
        \item $(\msg_0,\msg_1, st) \leftarrow A(1^\lambda, \ek)$ where $|\msg_0|=|\msg_1|=n$
        \item $|\ct\rangle \leftarrow \Enc(\ek, \msg_b)$
        \item $\rho^{BC} \leftarrow A(|\ct\rangle, st)$
        \item $\dk_0 \leftarrow \Keygen_2(1^\lambda, r_0)$, $\dk_1 \leftarrow \Keygen_2(1^\lambda, r_1)$, sample $d\leftarrow \bin$.
        \item $b_B \leftarrow B(\rho^B, \dk_d)$ and $b_C \leftarrow C(\rho^C, \dk_{1-d})$   where $B$ and $C$ are not allowed to communicate. 
    \end{enumerate}
    Concretely in our scheme we split the algorithm as follows:
    
    \begin{itemize}
        \item $\Keygen_1(1^\lambda, r)\rightarrow \ek$: $\Keygen_1$ uses randomness $r = (r_0,r_1)$ to run the $\Setup$ of the $\QFE$ scheme to obtain $(\mpk_0, \mpk_1,\msk_0,\msk_1)$ and outputs $\ek = (\mpk_0,\mpk_1)$.
        \item $\Keygen_2(1^\lambda,r_i)\rightarrow \dk$: $\Keygen_2$ uses the first part of the randomness to recreate $(\mpk_0, \mpk_1,\msk_0, \msk_1)$ and uses the second part of the randomness to define $(a,b)$ and creates the decryption key $\dk = (\sk_{C_0},\dk_{C_1})$, where $\sk_{C_j} \leftarrow \QFE.\Keygen(\msk_j, C_{a,b})$ for $j \in \bin$.
    \end{itemize}

    \begin{claim}
        Hybrid 0 and Hybrid 1 are perfectly indistinguishable.
    \end{claim}
    \begin{proof}
            This change is only syntactical and therefore the Hybrids are indistinguishable. 
    \end{proof}

    \paragraph{Hybrid 2:} In this Hybrid we change the encryption of $|\ct_0\rangle$ and the creation of $\dk_0$ as follows:
    \begin{itemize}
        \item $\Enc(\mpk, \msg)\rightarrow |\ct_\rangle$
        \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Create $|\ct_3\rangle$ as before: $|\ct_3\rangle  = \UEQ.\Enc(\ek',\msg)$, $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$.
        \item Create another copy of the decryption key $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$, where $|\dk_0\rangle = |\dk_1\rangle$ due to the pseudorandomness property of $\UEQ$.
        \item Sample $a_0,b_0,a_1,b_1,a'_0,b'_0,a'_1,b'_1 \in \bin^{l(\lambda)}$ randomly and create 
        $$ |\ct_0\rangle = \QFE.\Enc(\mpk_0, X^{a'_0} Z^{b'_0} |\dk_0\rangle, a_0, b_0, 1)$$.
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk_1, X^{a_1} Z^{b_1} |\dk_1\rangle ,a_1, b_1, 0)$$.


\iffalse
        \item Sample $d \leftarrow \bin$.
        \item Sample $l(\lambda)$ EPR pairs $\sigma^{AB}$. Let $\sigma^A$  denote  registers containing the first qubit of each EPR pair and $\sigma^B$ denote registers containing the second qubit of each EPR pair respectively.  Sample $a_0,b_0,a_1,b_1$ randomly and create the QFE ciphertexts:
        \item If $d = 0$ create 
        $$ |\ct_0\rangle = \QFE.\Enc(\mpk_0, \sigma_0^A, a_0, b_0, 1)$$.
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk_1, I/2 ,a_1, b_1, 0)$$.
        
        and teleport the key $|\dk_0\rangle$ through the EPR pairs $\sigma^B$ and obtain the teleportation keys $(a',b')$ and sample $a,b \leftarrow \bin^{l(\lambda)}$.
        \item If $d=1$ create 
        $$ |\ct_0\rangle = \QFE.\Enc(\mpk_0, \sigma_0^A, a_0, b_0, 1)$$.
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk_1, X^{a_1} Z^{b_1} |\dk\rangle ,a_1, b_1, 0)$$.
        and sample $(a,b),(a',b')$ $a,b, a',b' \leftarrow \bin^{l(\lambda)}$.
    \fi  
    \end{enumerate}
  
    \item Sample $d\leftarrow \bin$
    \item Set $r_d = (a_0', b_0')$ and set $r_{1-d} = (a'_1,b'_1)$.
.    \item $\Keygen_2(1^\lambda, (r,r_d)) \rightarrow \dk_d$: Create function secret keys for the circuit $C_{(a_0',b_0')}$ and output $\dk_d = (\sk_{C_0},\sk_{C_1})$.
    \item $\Keygen_2(1^\lambda, (r,r_{1-d})) \rightarrow \dk_{1-d}$: Create function secret keys for the circuit  $C_{(a_1',b_1')}$ and output $\dk_{1-d} = (\sk_{C_0},\sk_{C_1})$.
    \end{itemize}

    \begin{claim}
    \label{qfe:claim:hyb2qfered}
         Hybrid 1 and Hybrid 2 are computationally indistinguishable due to the single-key non-adaptive security of QFE. 
    \end{claim}

   \begin{proof}
       
  

    We show that an adversary $\Adv = (A, B, C)$ that can distinguish Hybrid 1 and Hybrid 2 can be used to break the security of the underlying $\QFE$ scheme. 

    Let $\Adv^*$ be the adversary in the single-query non-adaptive IND-security game (\cref{qfe:def:indsecurity}) against the quantum functional encryption scheme. $\Adv^*$ receives one public key $\mpk_0$ from the experiment creates the setup of the second QFE scheme $(\mpk_1, \msk_1) \leftarrow \QFE.\Setup(1^\lambda)$ and runs $A$ on input $(1^\lambda, (\mpk_0, \mpk_1))$ until $A$ outputs messages $\msg_0,\msg_1$. 
    To create the challenge message $\rho_{\msg^*_0}$ $\Adv^*$ performs the steps of the honest $\Enc$ algorithm (using randomness $r^*$ for $\UEQ.\Keygen$) without the creation of the $\QFE$ ciphertext $|\ct_0\rangle$. Then $\Adv^*$ sets

    $$\rho_{\msg_0^*} = X^{a_0} Z^{b_0} |\dk_0\rangle \otimes |a_0,b_0,0\rangle \langle a_0,b_0,0|$$ 
    To create the challenge message $\rho_{\msg^*_1}$ $\Adv^*$ performs the steps of $\Enc$ (using the same randomness $r^*$ for $\UEQ.\Keygen$ to recreate $|\dk_0\rangle$) as in Hybrid 2 without creation of the $\QFE$ ciphertext. That means $\Adv^*$ creates $l(\lambda)$ EPR pairs $\sigma^{AB}$ and teleports $\dk_0\rangle$ trough $\sigma^B$. Let $(a'_0,b'_0)$ be the resulting teleportation keys. Then, $\Adv^*$ sets: 

    $$ \rho_{\msg_1^*} = \sigma_0^A \otimes |a_0,b_0,1\rangle\langle a_0,b_0,1|$$

    Note that in this message the flag bit $c$ is set to $1$.
    Now $\Adv^*$ defines $(\rho_{\msg_0^*}, \rho_{\msg_1^*})$ as challenge messages. 
    $\Adv^*$ requests a function secret key $\sk_C$ for the circuit $C_{(a'_0, b'_0)}$. The combination of message and key queries is an admissible query, since 

    $$C_{(a'_0, b'_0)}(\rho_{\msg_0^*}) = |\dk_0\rangle = C_{(a'_0, b'_0)}(\rho_{\msg_1^*}) $$
    and $\Adv^*$ is not entangled with the state. 

    $\Adv^*$ receives $\rho_{\ct}$ from the experiment finishes the simulation of the experiment by forwarding $(\rho_{\ct}, |\ct_2\rangle, |\ct_3\rangle)$ to $A$, where $|\ct_2\rangle$ and $|\ct_3\rangle$ are created as in the honest encryption algorithm, Hybrid 1 and Hybrid 2 do not differ in this aspect. Then $\Adv^*$ creates the secret key $\sk_{C_1} \leftarrow \QFE.\Keygen(1^\lambda, \msk_1, C_{(a_1,b_1)})$ for random $a,b \leftarrow \bin^{l(\lambda)}$. $\Adv^*$ receives $\rho^{BC}$, forwards $(\rho^B,\sk_C)$ to $B$ and $(\rho^C, \sk_{C_1})$ to $C$. The simulation corresponds to Hybrid 1 if the IND-security experiment for QFE selected $\rho_{m_0^*}$ as challenge message and the simulation corresponds to Hybrid 2 if the IND-security experiment for QFE selected $\rho_{m_1^*}$ as challenge message. Therefore, if $(A,B,C)$ can distinguish the Hybrids, $\Adv^*$ can break the non-adaptive single-key security of $\QFE$.
 \end{proof}

    \paragraph{Hybrid 3:} In this Hybrid we change the encryption of $|\ct_1\rangle$ and the creation of $\dk_1$ as follows:
    \begin{itemize}
        \item $\Enc(\mpk, \msg)\rightarrow |\ct_\rangle$
        \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Create $|\ct_3\rangle$ as before: $|\ct_3\rangle  = \UEQ.\Enc(\ek',\msg)$, $(\ek',|\dk_0\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$, $(\ek',|\dk_1\rangle) \leftarrow \UEQ.\Keygen(1^\lambda, r^*)$
        \item Sample $l(\lambda)$ EPR pairs $\sigma^{AB}$. Let $\sigma^A$  denote  registers containing the first qubit of each EPR pair and $\sigma^B$ denote registers containing the second qubit of each EPR pair respectively.  Sample $a_1,b_1$ randomly and create the QFE ciphertext 
        $$ |\ct_1\rangle = \QFE.\Enc(\mpk,\sigma_1^A,a_1,b_1,1)$$.
        \item Create $|\ct_0\rangle$ as in Hybrid 2.% which gives $(a_0',b_0')$ .
        
        
        \item Teleport the key $|\dk_1\rangle$ through the EPR pairs $\sigma^B$ and obtain the teleportation keys $(a_1',b_1')$.
    \end{enumerate}
    \item Set $r_{1} = (a_0,b_0,a_{1}',b'_{1},1)$ for $a_0,b_0 \leftarrow \bin^{l(\lambda)}$.
    \item $\Keygen_2(1^\lambda, (r,r_1)) \rightarrow \dk_1$: Create a function secret key for the circuit  $C_{(a_{1}',b_{1}')}$.
    \item Create $|\dk_0\rangle$ as in Hybrid 2.
    
    \end{itemize}
    

    \begin{claim}
        Hybrid 2 and Hybrid 3 are computationally indistinguishable due to the single-key non-adaptive security of QFE.
    \end{claim} 
    \begin{proof}
        The proof follows the same argument as the proof for the previous claim so we omit it here.
    \end{proof}
    
    
    \begin{lemma}
        In Hybrid 3 the advantage of $\Adv = (A, B, C)$ is negligible if UEQ fulfills uncloneable security for UE schemes with quantum decryption keys (\cref{qfe:def:ueqsec}).
    \end{lemma}
\begin{proof}
    We show that an adversary that breaks the security of the uncloneable encryption scheme breaks uncloneability of the underlying $\UEQ$ encryption scheme with quantum decryption keys with the same advatage. 

    Let $(A,B,C)$ be an adversary that breaks the security of the uncloneable encryption scheme. Then we can build an adversary $(A^*, B^*, C^*)$ that breaks the security of the $\UEQ$ scheme. Run the $\Keygen_1(1^\lambda)$ algorithm to obtain $\ek$  and run $A$ on input $(1^\lambda, \ek)$. Receive the challenge messages $\msg_0, \msg_1$ from $A$ and forward the messages to the experiment of $\UEQ$. Receive the challenge ciphertext $|\ct\rangle$. 
    
    Build the ciphertext as in Hybrid 3: Sample 2 sets of n EPR pairs $\sigma_0^{AB}$ and $\sigma_1^{AB}$. Let $\sigma_0^A$, $\sigma_1^A$ denote registers containing the first qubit of each EPR pair and $\sigma_0^B$,$\sigma_0^B$ denote registers containing the second qubit of each EPR pair respectively. Sample $a_0,b_0,a_1,b_1 \leftarrow \bin^{l(\lambda)}$ and create the ciphertexts 
    
    $$|\ct_0 \rangle = \QFE.\Enc(\mpk,\sigma_0^A, a_0,b_0,1)$$ 
    $$|\ct_1 \rangle = \QFE.\Enc(\mpk,\sigma_1^A, a_1,b_1,1) $$
    
    and send $(|\ct_0\rangle, |\ct_1\rangle, |\ct\rangle)$ to  $A$. 
    
    
    $A$ performs the splitting channel and outputs a state $\rho^{BC}$ which is also the state that $A^*$ defines as it's result of the splitting channel. 
    Now $B^*$ and $C^*$ are activated. They take as input the states ($\rho^B, \sigma_0^B$) and ($\rho^C, \sigma_1^B$) respectively and each receive a copy of the secret key $|\dk\rangle$ from the experiment. 


    $B^*$ teleports the state $|\dk\rangle$ trough the EPR pairs $\sigma_0^B$ and obtains the teleportation correction keys $a'_0,b'_0$. He produces the secret key $\dk_B = \QFE.\Keygen(\msk, C_{(a'_0,b'_0)})$. He runs the adversary $B$ on input $\rho^B$ and the secret key ($\dk_B$,0) and outputs whatever $B^*$ outputs. 

    $C^*$ does the same actions as $B^*$ on his respective EPR pairs. He teleports the state $|\dk\rangle$ trough the EPR pairs $\sigma_1^B$. He obtains the teleportation correction keys $a'_1,b'_1$ and produces the secret key $\dk_C = \QFE.\Keygen(\msk, C_{(a'_1,b'_1)})$. He runs the adversary $C$ on input $\rho^C$ and the secret key ($\dk_C$,1) and outputs whatever $C^*$ outputs. 
    
    $(A^*, B^*, C^*)$ wins with the same probability as $(A,B,C)$. 
\end{proof}
\end{proof}

\paragraph{Remark} Can we use \cite{HKNY23} to make the single bit uncloneable encryption scheme into a multi-bit uncloneable encryption scheme?. 

\paragraph{Remark} Mention that the independently sampled decryption keys security notion is still useful for public key quantum money.
    
\end{comment}

\subsection{realted work}
related work uncloneable encryption:
\begin{itemize}
    \item \cite{AKY24} construct indistinguishable uncloneable secure encryption, first scheme that achieves this in plain model but with quantum secret keys
    \item \cite{C:AKLLZ20} On the Feasibility of Unclonable Encryption, and More
    \begin{enumerate}[align=left, leftmargin=2.8em]
        \item Build indistinguishable-uncloneable encryption in the QROM
        \item Show that a certain class of uncloneable encryption scheme cannot exist: If Enc is a unitary $U$ and Dec is a unitary $U^\dag$. But that is not the case in our scheme.
        \item TODO Read 
    \end{enumerate}
    \item \cite{BC23} uncloneable encryption with interaction TODO read
    \item \cite{TCC:AnaKal21} transform one-time uncloneable encryption scheme into multi message private key or public key encryption scheme. 
    \item \cite{HKNY23} Extending length of plaintext in UE
    \item KT23 Device-independent uncloneable encryption
\end{itemize}


